Passive Heart Rate Monitoring During Smartphone Use in Everyday Life

Resting heart rate (RHR) is an important biomarker of cardiovascular health and mortality, but tracking it longitudinally generally requires a wearable device, limiting its availability. We present PHRM, a deep learning system for passive heart rate (HR) and RHR measurements during everyday smartphone use, using facial video-based photoplethysmography. Our system was developed using 225,773 videos from 495 participants and validated on 185,970 videos from 205 participants in laboratory and free-living conditions, representing the largest validation study of its kind. Compared to reference electrocardiogram, PHRM achieved a mean absolute percentage error (MAPE) < 10% for HR measurements across three skin tone groups of light, medium and dark pigmentation; MAPE for each skin tone group was non-inferior versus the others. Daily RHR measured by PHRM had a mean absolute error < 5 bpm compared to a wearable HR tracker, and was associated with known risk factors. These results highlight the potential of smartphones to enable passive and equitable heart health monitoring.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> removed.tex <==
\begin{wraptable}{r}{8cm}
    \centering
    \caption{\textbf{Downstream Datasets.} Downstream dataset states.}
    \begin{tabular}{rcc}
    \toprule
        \textbf{Class}   & \textbf{\# Training} & \textbf{\# Testing} \\
        \midrule
        Exercise & 3,272 & 671\\
        Non-Exercise & 6,195 & 1,329 \\
        \hdashline
        %Aerobics & xxx & xxx. \\ 
        Biking & 1,191 & 412 \\ 
        %Core training & xxx & xxx. \\ 
        Elliptical & 152 & 49 \\ 
        High Intensity Int. Training & 332 & 104 \\ 
        Hiking & 561 & 65 \\ 
        %Paddleboarding & xxx & xxx. \\ 
        %Pilates & xxx & xxx. \\ 
        %Rowing & xxx & xxx. \\ 
        %Running Outdoor & xxx & xxx. \\ 
        %Spinning & xxx & xxx. \\ 
        Strength training & 229 & 425 \\  
        Swimming & 2,332 & 441 \\ 
        Running (Non-Treadmill) & 1,860 & 315 \\ 
        Running (Treadmill) & 159 & 52 \\ 
        Walking & 6,887 & 1,301 \\ 
        Weightlifting & 669 & 98 \\ 
        %Yoga & xxx & xxx. \\ 
        %Zumba & xxx & xxx. \\ 
        \bottomrule
        \end{tabular}
    \label{tab:downstream_classification}
\end{wraptable}



\begin{wraptable}{r}{9cm}
\centering
\caption{\textbf{Demographics.} Gender, age and body-mass index of our pretraining sample. } \label{tab:demographics}
    \sisetup{group-four-digits}
    \renewcommand\tabularxcolumn[1]{m{#1}}
    \small
\begin{tabularx}{0.8\linewidth}{@{}
                    L 
                    c]
               c}
        \toprule
Category 
    & {\makecell[b]{\# Individuals}}
        & {\makecell[b]{Percentage}}
                     \\ 
    \midrule
\textbf{Gender} \\
\quad Female & 110,780 & 67.0\% 
        \\ 
\quad Male & 53,895 & 32.6\% \\
\quad Not Specified & 415 & 0.3\% 
        \\ \addlinespace[2pt]
\textbf{Age} \\
\quad 18-39     & 55,653 & 33.7\% \\
\quad 40-59     & 75,627 & 45.8\% \\  
\quad 60-79     & 32,251 & 19.5\% \\  
\quad 80+       & 1,548 & 0.9\% \\  
\addlinespace[2pt]
\textbf{BMI} \\
\quad Healthy ($<$25)   & 57,015 & 34.5\% \\
\quad Overweight (25-30)   & 52,950 & 32.0\% \\
\quad Obese (30+)   & 54,727 & 33.1\% \\
\quad Not Specified   & 575 & 0.3\% \\
 \addlinespace[2pt]  \bottomrule %
\end{tabularx}
\end{wraptable}





\begin{table}[h]
    \centering
    \caption{\textbf{Results}}
    \begin{tabular}{lcccccc}
    \toprule
        \textbf{Task + Method} & \multicolumn{6}{c}{\textbf{Performance}} \\
        \midrule
        \grayrow 
        & \multicolumn{2}{c}{\textbf{30 mins}} & \multicolumn{2}{c}{\textbf{60 mins}} & \multicolumn{2}{c}{\textbf{120 mins}} \\
        \grayrow 
        \multirow{-2}{*}{\textbf{Signal Imputation}} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} \\
        \midrule
         Mean & 0.37 & 0.44 & 0.38 & 0.46 & 0.39 & 0.49 \\
         Nearest Neighbor & 0.28 & 0.42 & 0.33 & 0.51 & 0.38 & 0.62 \\
         Linear Interpolation & 0.26 & 0.34 & 0.30 & 0.42 & 0.36 & 0.51 \\
         LSM (Ours) & ... \\[1.2pt]

        \midrule
        \grayrow 
        & \multicolumn{2}{c}{\textbf{30 mins}} & \multicolumn{2}{c}{\textbf{60 mins}} & \multicolumn{2}{c}{\textbf{120 mins}} \\
        \grayrow 
        \multirow{-2}{*}{\textbf{Signal Forecasting}} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} \\
        \midrule
         Mean & 0.47 & 0.65 & 0.47 & 0.64 & 0.45 & 0.64 \\
         Nearest Neighbor & 0.43 & 0.68 & 0.47 & 0.76 & 0.48 & 0.81 \\
         Linear Interpolation & 0.43 & 0.68 & 0.47 & 0.76 & 0.48 & 0.81 \\
         PatchTST~\cite{} \\
         TIDE~\cite{} \\
         NBEATS~\cite{} \\
         Moment(?)~\cite{} \\
         LSM (Ours) & \\[1.2pt]
        
        \midrule
        \grayrow
        \multicolumn{1}{l}{\textbf{Exercise Classification}} & \ \textbf{Acc.} & \textbf{mAP} & \textbf{Others???} &&& \\
        \midrule
         ResNet18 & ... \\
         ViT-B & ... \\
         LSM + Linear Probe (Ours) & ... \\
         LSM + Fine-tuning (Ours) & ... \\

         \midrule
        \grayrow
        \multicolumn{1}{l}{\textbf{Stress Classification}} &&&&&& \\
        \midrule
         ResNet18 & ... \\
         ViT-B & ... \\
         LSM + Linear Probe (Ours) & ... \\
         LSM + Convolution Probe (Ours) & ...\\
         LSM + Fine-tuning (Ours) & ... \\
         
        \midrule
        \grayrow
        \multicolumn{1}{l}{\textbf{Exercise vs Mood Event Classification}} &&&&&& \\
        \midrule
         ResNet18 & ... \\
         ViT-B & ... \\
         LSM + Linear Probe (Ours) & ... \\
         LSM + Convolution Probe (Ours) & ...\\
         LSM + Fine-tuning (Ours) & ... \\

        \bottomrule
        \end{tabular}
    \label{tab:downstream_task_results}
\end{table}













\subfloat[][\textbf{Demographics.} Gender, age and body-mass index of our pretraining sample. ]{
\centering
\label{tab:demographics}
\begin{tabular}{rcc}
\toprule
\textbf{Category}
& {\makecell[b]{\textbf{\# People}}}
& {\makecell[b]{\textbf{\%}}} \\ 
\midrule
%\textbf{Gender} \\
\textbf{Gender} \quad \quad \quad Female & 110,780 & 67.0\%  \\ 
\quad Male & 53,895 & 32.6\% \\
\quad Not Specified & 415 & 0.3\%  \\ \addlinespace[4pt]
%\textbf{Age} \\
\textbf{Age} \quad \quad \quad \quad \quad 18-39     & 55,653 & 33.7\% \\
\quad 40-59     & 75,627 & 45.8\% \\  
\quad 60-79     & 32,251 & 19.5\% \\  
\quad 80+       & 1,548 & 0.9\% \\  
\addlinespace[4pt]
%\textbf{BMI} \\
\textbf{BMI} \quad Healthy ($<$25)   & 57,015 & 34.5\% \\
\quad Overweight (25-30)   & 52,950 & 32.0\% \\
\quad Obese (30+)   & 54,727 & 33.1\% \\
\quad Not Specified  & 575 & 0.3\% \\
\hdashline
\quad \textbf{Total} & 165,090 & 100\% \\
 \addlinespace[4pt]  \bottomrule %
\end{tabular}}
\quad
\subfloat[][\textbf{Downstream Dataset.} Class distributions for downstream exercise and activity classification.]
{\centering
    \begin{tabular}{rcc}
    \toprule
        \textbf{Class}   & \textbf{\# Training} & \textbf{\# Testing} \\
        \midrule
        Exercise & 3,272 & 671\\
        Non-Exercise & 6,195 & 1,329 \\
        \hdashline
        %Aerobics & xxx & xxx. \\ 
        Biking & 1,191 & 412 \\ 
        %Core training & xxx & xxx. \\ 
        Elliptical & 152 & 49 \\ 
        High Intensity Train & 332 & 104 \\ 
        Hiking & 561 & 65 \\ 
        %Paddleboarding & xxx & xxx. \\ 
        %Pilates & xxx & xxx. \\ 
        %Rowing & xxx & xxx. \\ 
        %Running Outdoor & xxx & xxx. \\ 
        %Spinning & xxx & xxx. \\ 
        Strength training & 229 & 425 \\  
        Swimming & 2,332 & 441 \\ 
        Running & 1,860 & 315 \\ 
        Running (Treadmill) & 159 & 52 \\ 
        Walking & 6,887 & 1,301 \\ 
        Weightlifting & 669 & 98 \\ 
        \hdashline
        \textbf{Total} & \\ 
        %Yoga & xxx & xxx. \\ 
        %Zumba & xxx & xxx. \\ 
        \bottomrule
        \end{tabular}}
\end{table}














\begin{table}[h]
    \centering
    \caption{\textbf{Generative Task Results}}
    \begin{tabular}{lccc}
    \toprule
        \textbf{Task + Method} & \multicolumn{3}{c}{\textbf{Error (MAE / MSE)}} \\
        \midrule
        \grayrow 
        \textbf{Signal Imputation}  & \textbf{30 mins} & \textbf{60 mins} & \textbf{120 mins} \\
        \midrule
         Mean & 0.37 / 0.44 & 0.38 / 0.46 & 0.39 / 0.49 \\
         Nearest Neighbor & 0.28 / 0.42 & 0.33 / 0.51 & 0.38 / 0.62 \\
         Linear Interpolation & 0.26 / 0.34 & 0.30 / 0.42 & 0.36 / 0.51 \\
         LSM (Ours) & \textbf{0.20} / \textbf{0.21} & \textbf{0.24} / \textbf{0.26} & \textbf{0.29} / \textbf{0.33} \\[1.2pt]
        \midrule
        \grayrow 
        \textbf{Signal Forecasting} & \textbf{30 mins} & \textbf{60 mins} & \textbf{120 mins} \\
        \midrule
         Mean & 0.47 / 0.65 & 0.47 / 0.64 & 0.45 / 0.64 \\
         Nearest Neighbor & 0.43 / 0.68 & 0.47 / 0.76 & 0.48 / 0.81 \\
         Linear Interpolation & 0.43 / 0.68 & 0.47 / 0.76 & 0.48 / 0.81 \\
         %PatchTST~\citep{} \\
         %TIDE~\citep{} \\
         %NBEATS~\citep{} \\
         %Moment(?)~\citep{} \\
         LSM (Ours) & \textbf{0.34} / \textbf{0.40} & \textbf{0.37} / \textbf{0.44} & \textbf{0.38} / \textbf{0.47}\\ \bottomrule[1.2pt]
        \end{tabular}
    \label{tab:downstream_task_results}
\end{table}





\begin{table}[h]
    \centering
    \caption{\textbf{Classification Task Results.}}
    \begin{tabular}{lcc}
    \toprule       
        \grayrow
        \textbf{Exercise Classification} & \textbf{Acc.} & \textbf{mAP} \\
        \midrule
        \midrule
         ResNet18 & 56.6 & 21.4  \\
         ResNet50 & 60.4 & 27.5  \\
         ResNet200 & 63.9 & 29.7  \\
         ViT-B & ... \\
         LSM + Linear Probe (Ours) & 49.5 & 19.8  \\
         LSM + Conv. Probe (Ours) & \textbf{69.0} & 36.5 \\
         LSM + Fine-tune (Ours) & 68.5 & \textbf{36.7}  \\

      %   \midrule
      %  \grayrow
      %  \multicolumn{1}{l}{\textbf{Stress Classification}} &&&&&& \\
      %  \midrule
      %   ResNet18 & ... \\
      %   ViT-B & ... \\
      %   LSM + Linear Probe (Ours) & ... \\
      %   LSM + Convolution Probe (Ours) & ...\\
      %   LSM + Fine-tuning (Ours) & ... \\
         
        \midrule
        \grayrow
        \textbf{Stress Classification} & \textbf{Acc.} & \textbf{mAP}  \\
        \midrule \midrule
         ResNet18 & ... \\
         ViT-B & ... \\
         LSM + Linear Probe (Ours) & ... \\
         LSM + Conv. Probe (Ours) & ...\\
         LSM + Fine-tune (Ours)  \\

        \bottomrule[1.2pt]
        \end{tabular}
    \label{tab:downstream_task_results}
\end{table}
